Learning for Multi-robot Cooperation in Partially Observable Stochastic Environments with Macro-actions

This paper presents a data-driven approach for multi-robot coordination in partially-observable domains based on Decentralized Partially Observable Markov Decision Processes (Dec-POMDPs) and macro-actions (MAs). Dec-POMDPs provide a general framework for cooperative sequential decision making under uncertainty and MAs allow temporally extended and asynchronous action execution. To date, most methods assume the underlying Dec-POMDP model is known a priori or a full simulator is available during planning time. Previous methods which aim to address these issues suffer from local optimality and sensitivity to initial conditions. Additionally, few hardware demonstrations involving a large team of heterogeneous robots and with long planning horizons exist. This work addresses these gaps by proposing an iterative sampling based Expectation-Maximization algorithm (iSEM) to learn polices using only trajectory data containing observations, MAs, and rewards. Our experiments show the algorithm is able to achieve better solution quality than the state-of-the-art learning-based methods. We implement two variants of multi-robot Search and Rescue (SAR) domains (with and without obstacles) on hardware to demonstrate the learned policies can effectively control a team of distributed robots to cooperate in a partially observable stochastic environment.

==> sar.tex <==
\subsection{Search and Rescue Problem}\label{app:sar}

%%% math
%\usepackage{amsmath}
%\usepackage{amssymb}
%

Our search and rescue problem involves a heterogeneous set of autonomous agents searching for victims after a disaster and rescuing survivors (e.g., bringing them to a location where medical attention can be provided). Due to communication limitations, each agent has to make decisions based on their limited information gathered from their observations and communications. The agents need to decided how to explore the environment and how to prioritize victims that they discover.

%\subsection{Problem Description}

The scenario begins after a natural disaster strikes the simulated world. Throughout the world there are $s$ sites. At each site, there may be injured victims with varying initial levels of critically. Each victim's health degrades with time. We want to retrieve as many victims as we can and bring them to the muster area before they die.  An autonomous air vehicle (e.g., unmanned helicopter) surveys the disaster from above.  A set of autonomous ground vehicles can search the space or retrieve victims and deliver them to the muster site, where medical attention is provided. 

The objective of the team is maximize the number of victims returned to the muster site while they are still alive.

The search and rescue domain we consider is a 20 $\times$ 10 unit grid with 6 designated sites - 1 muster site and 5 victim sites. All agents are initialized at the muster site. Victim sites are randomly populated with victims (6 victims total). Each victim has an associated initial health value, which is also randomly initialized. While the locations of the sites are known, the number of victims and their health at each site is unknown to the agents. The maximum victim capacity of each site varies based on the site size. Agents conduct collision avoidance and obstacles are scattered throughout the environment to embed additional uncertainty into the domain. 

	There are 4 agents in total, 1 unmanned aerial vehicle (UAV) and 3 unmanned ground vehicles (UGVs). In this domain, only the UGVs can carry victims, while only the UAV can observe victims. All agents have 6 macro-actions which allow them to navigate to each site. The UGV has an extra macro-action allowing victim pickup. \sXX{do UGVs automatically drop victims if they go to muster, or is there a separate MA for that?} \kXX{yes they automatically drop victims when they go to muster}
    
	In each scenario, a robot can observe its own location, whether there are victims at that location, and the health of a present victim \sXX{specify more details about these observations - are they binary/discrete/continuous/what's their range/etc,}. All observations have noise that is distributed uniformly \sXX{this is somewhat unclear, distributed uniformly can mean a lot of things. For a discrete variable, what does that mean? For a continuous variable, discreted uniformly doesn't make sense unless the support of that distribution is provided.}. Robots within a certain proximity to each other can also communicate to each other, updating values in their observation matrices \sXX{matrices or vectors?} based on the most recent observations taken between the two agents \sXX{bit unclear how this update is done - sentence might need to be reworded}.
    
	The objective for the agents is to rescue all 6 victims by transporting them back to the muster before any of them die either at their site locations or on the way to the muster. The reward for rescuing a victim is +1, so the maximum value possible (given no discounting) is 6.

\subsection{Simulator Description}
The simulator executes a time-stepped model of the scenario.  Scenario parameters define the map of the world, number of each type of agent, and locations and initial states of victims.

Each agent's macro-controller policy is executed by a lower-level controller which checks the initiation and termination conditions for the macro-action and generates sequences of primitive actions.

\subsubsection{Primitive Actions}
The simulator models primitive actions, each of which take one time step to execute.  The primitive actions for the agents are:
\begin{itemize}
\item move vehicle,
\item pick-up victim (ground agents only),
\item drop-off victim (ground agents only), and
\item do nothing.
\end{itemize}

Observations and communication occur automatically whenever possible and do not take any additional time to execute.

Macro-action policies, built from these primitive actions, may take any arbitrary amount of time in multiples of the time-step of the simulator.

\subsubsection{The World}
The world is modeled as a two-dimensional plane divided into an evenly-spaced grid within a rectangular boundary of arbitrary size.\mXX{The robot implementation is in 3D, are there any technique challenge worth mentioning?}  Each rescue site is a discrete rectangle of grid spaces of arbitrary size within the world.

Some number of victims are initially located in the rescue sites.  Victim health is represented as a value from 0 to 1, with 1 being perfectly healthy and 0 being dead.  Each victim may start at any level of health, and its health degrades linearly with time.  If a victim is brought to the muster location, its health goes to 1 and no longer degrades.  One victim at a time may be transported by a ground agent to the muster.\mXX{We can generalize this by allowing taking multiple victims at a time}

\subsubsection{Movement}
Simple kinematic models are used to represent the motion of the air and ground vehicles.  The vehicles can move within the rectangular boundaries of the world defined in the scenario.

The ground vehicle motion is modeled with constant speed in one of the four cardinal directions, and instantaneous acceleration.  Any obstacles in the world, including other ground vehicles, must be navigated around.  The ground vehicle uses a wall-following technique to get around obstacles.\mXX{This is not a good technique, how is it done for real robot? Need to mention the real implementation of low level control.} In the event that the ground vehicle is stuck, it will perturb its path by moving one step in a random direction.\mXX{We are using RVO now, right?}

The air vehicle is modeled with an approximately constant speed in any direction, and instantaneous acceleration\mXX{This is not true for real robot. Since we have a simulator in ROS, maybe we should mention that instead}.  Since the air vehicle model represents a vehicle that is operating at a higher altitude than the ground vehicles and obstacles, there are no restrictions to the air vehicle's movement.\mXX{Is is true the the simulator in ROS as well?}\sXX{kavin, does the UAV also avoid obstacles?}

For the scenarios used to generate the results in this study, the ground vehicle can move exactly one grid space in one time-step of the simulator and the air vehicle moves approximately 5x faster.

\subsubsection{Observations}
In the scenario, an air agent can observe victim locations when over a rescue site.  Victim health status is not observable by air.  A ground agent that is in a rescue site can observe all victims (location and health status) within that site.  Agents are always able to observe their own location and a victim they are holding.  Observations are imperfect; observations have a .05 probability of being inaccurate.

\subsubsection{Communication}
Communication is range-limited.  When agents are within range (which is larger for UAV-UGV communication than for UGV-UGV communication), they will automatically share their observations with two-way communication.  Communication is imperfect; communication has a .05 probability of failing to occur even when agents are in range.

For the scenarios used to generate the results in this study, the ground vehicles can communicate with any other ground vehicles within 3 grid spaces in any direction; the air vehicles can communicate with any ground vehicles or other air vehicles within 6 grid spaces in any direction.

\subsection{MacDec-POMDP Representation}

Each agent has a set of macro-actions that can be executed by the agent's decentralized policy at each decision epoch. The macro-action is executed by a lower level controller of primitive actions.  The macro-actions for each ground agent are:
\begin{itemize}
\item Go to muster and drop off victims,
\item Pick up victim at current site,
\item Go to site $i \in \{1,\ldots,s\}$
\end{itemize}
The macro-actions for each air agent are:
\begin{itemize}
\item Go to site $i \in \{1,\ldots,s\}$ 
\end{itemize}


\subsubsection{Rewards}

The reward is $+1$ for each victim brought back to muster alive and $-1$ for each victim who dies.

\subsubsection{Observation Vectors}

The observation vector $O$ on which the macro-controller makes decisions is a subset of the raw observations each agent may have accumulated through the execution of the prior macro-action.  The agents report the state of their current location and one other location (which could be directly observed or received via communication while completing the macro action).  The second location reported is the most urgent state with the most recent new observation.  If there are no new observations other than the agent’s own location, then the second location will be equal to the self location.

The disaster area is divided into a discrete set of rescue ``sites,'' conceptually areas in which victims may be located.  The map is represented as a 2-dimensional horizontal plane.\mXX{Refer to a picture in ROS visualization tool?.}

Observations are according to
\begin{equation}
 O = 
\begin{bmatrix}
\text{self state} \\
\text{self location} \\
\text{location state} \\
\text{second location} \\
\text{second location state} \\
\end{bmatrix} \,,
\end{equation}
where
\begin{itemize}
\item self state $\in$ \{0=not holding victim, 1=holding victim\},
\item self location $\in$ \{site 1, site 2, ..., site s\},
\item location state $\in$ \{0=no victims needing help, 1=victims needing help (not critical), 2=critical victims\},
\item second location $\in$ \{site 1, site 2, ..., site s\}, and
\item second location state $\in$ \{0=no victims needing help, 1=victims needing help (not critical), 2=critical victims\}.
\end{itemize}
Note that there are $18s^2$ possible observation vectors.\mXX{Is this a challenge for G-DICE or other planning based methods?}

\subsubsection{Macro Action Descriptions}

More detail about the macro-actions in this problem are as follows.
\begin{itemize}
\item \textbf{Go to Muster}: Agent tries to go to the muster point from anywhere else, but only if it is holding a live victim.  If a victim is on-board, victim will always disembark at the muster.\mXX{Is battery level considered in ROS simulator?}
\item \textbf{Pick up Victim}: Agent tries to go to a victim's location from a starting point within the site.  Terminates when the agent reaches the victim; also may terminate if there is no longer a victim needing help at the site (i.e. another agent picked the victim up first or the victim died).  If victim and agent are co-located in the same grid cell, the victim can be ``picked up''.
\item \textbf{Go to Site $x$}: Agent goes to a specified disaster site $x$.  Terminates when the agent is in the site.  Agent can get observations of the victims at the site.
\end{itemize}


%\subsection{Macro-Controller}

%The macro-controller is the finite-state machine policy which specifies the transition to the next macro-action.  The macro-controller is completely described by the Action Matrix and the Transition Matrix.

%The action matrix, A, is defined as
%$$A\{i\}(j)=k$$
%where $i$ is the agent index, 
%$j$ is the node index,
%and $k$ is the macro action index\\

%The transition matrix, T, is defined as
%$$T\{i,j\}=[k \;\;\; o]$$
%where $i$ is the agent index, 
%$j$ is the current node index, 
%$k$ is the next node index, 
%and $o$ is an observation vector\\


